Mixed-Precision Embedding Using a Cache

In recommendation systems, practitioners observed that increase in the number of embedding tables and their sizes often leads to significant improvement in model performances. Given this and the business importance of these models to major internet companies, embedding tables for personalization tasks have grown to terabyte scale and continue to grow at a significant rate. Meanwhile, these large-scale models are often trained with GPUs where high-performance memory is a scarce resource, thus motivating numerous work on embedding table compression during training. We propose a novel change to embedding tables using a cache memory architecture, where the majority of rows in an embedding is trained in low precision, and the most frequently or recently accessed rows cached and trained in full precision. The proposed architectural change works in conjunction with standard precision reduction and computer arithmetic techniques such as quantization and stochastic rounding. For an open source deep learning recommendation model (DLRM) running with Criteo-Kaggle dataset, we achieve 3x memory reduction with INT8 precision embedding tables and full-precision cache whose size are 5% of the embedding tables, while maintaining accuracy. For an industrial scale model and dataset, we achieve even higher >7x memory reduction with INT4 precision and cache size 1% of embedding tables, while maintaining accuracy, and 16% end-to-end training speedup by reducing GPU-to-host data transfers.

==> FIGURES/gpu/fig_gpu_speed.tex <==
\begin{figure}[h!]
\begin{tabular}{cc}
  \includegraphics[width=40mm]{FIGURES/gpu/lru_fwd_zipf.pdf} &   \includegraphics[width=40mm]{FIGURES/gpu/lru_bwd_zipf.pdf} \\
   {\small (a) LRU, forward} & {\small (b) LRU, backward} \\[6pt]
%  \includegraphics[width=40mm]{FIGURES/gpu/lfu_fwd.pdf} &  \includegraphics[width=40mm]{FIGURES/gpu/lfu_bwd.pdf} \\
% \small (c) LFU, forward} & {\small (d) LFU, backward} \\[6pt]
\end{tabular}
\caption{Effective bandwidth for FP32 vs. FP16 with full-precision cache}
\label{fig:gpu-speed}
\end{figure}
% [Remove the FP32 blue line as we didn't mentioned FP32 cache in the paper?]

==> gpu.tex <==
\section{GPU}

% TO Add more details by JH.
In this section, we give the details of the GPU implementation.


\subsection{Stochastic Rounding Implementation on GPUs}


\subsection{Set Associative Cache}



\subsection{High-precision Cache}


==> old_graphs.tex <==

\begin{figure}[h!]
\begin{tabular}{cc}
  \includegraphics[width=40mm]{FIGURES/cpu/lru-nearest-drop.png} &   \includegraphics[width=40mm]{FIGURES/cpu/lru-stoc-drop.png} \\
   (a) LRU nearest rounding & (b) LRU stochastic rounding \\[6pt]
 \includegraphics[width=40mm]{FIGURES/cpu/lfu-nearest-drop.png} &  \includegraphics[width=40mm]{FIGURES/cpu/lfu-stoc-drop.png} \\
(c) LFU nearest rounding & (d) LFU stochastic rounding \\[6pt]
\end{tabular}
\caption{High-precision LRU and LFU cache with varying cache sizes recover accuracy for low-precision embeddings
\Comment{PT: Help! really hard to read the ylabel and the descriptions on top of each of these 4 pictures}
}
\label{fig:cpu-lfu-lru}
\end{figure}


\begin{figure}[h!]
\begin{tabular}{cc}
  \includegraphics[width=40mm]{FIGURES/cpu/LRU-near-size.png} &   \includegraphics[width=40mm]{FIGURES/cpu/LRU-stoc-size.png} \\
   (a) LRU nearest rounding & (b) LRU stochastic rounding \\[6pt]
 \includegraphics[width=40mm]{FIGURES/cpu/LFU-near-size.png} &  \includegraphics[width=40mm]{FIGURES/cpu/LFU-stoc-size.png} \\
(c) LFU nearest rounding & (d) LFU stochastic rounding \\[6pt]
\end{tabular}
\caption{Diminishing return of accuracy recovery vs. cache sizes}
\label{fig:cpu-cache-size}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=3.2in]{FIGURES/cache_forward_pic.pdf}
    \caption{Forward pass involving a low-precision embedding table $T$ and a full-precision cache $C$}
    \label{fig:cache_forward_pass}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=2.5in]{FIGURES/cache_backward_pic.pdf}
    \caption{Backward pass involving a low-precision embedding table $T$ with a full-precision cache}
    \label{fig:cache_backward_pass}
\end{figure}


\begin{algorithm}
   \caption{Update with Set-Associative LFU Cache}
   \label{alg:cpu-assoc-lfu}
\begin{algorithmic}
   \STATE {\bfseries Input:} embedding $T$, sets of indices $I_C$ of current cached rows, indices to update $I_U$, hash function $h$, gradient update $U$, access counters $Q$ 
   \FOR{$i$ in $_U$}
   \STATE $Q[i] = Q[i] + 1$
   \IF{$i \in I_C[h(i)]$}
   \STATE apply gradient updates $T[i,:] = T[i,:] + U[i,:]$
   \ELSE 
     \STATE dequantize $T[i,:]$ (an no-op)
     \STATE and apply gradient updates $T[i,:] = T[i,:] + U[i,:]$
     \STATE get $s \gets h(i)$, 
     \STATE and $j$ such that $Q[j] = \min\{Q[k] | k \in I_C[s]\}$
     \IF{$Q[i] \le Q[j]$} 
     \STATE quick bypass as follows
     \STATE fake quantize $T[i,:]$
     \ELSE 
     \STATE fake quantize $T[j,:]$
     \STATE replace $j$ by $i$ in the set $I_C[s]$
     \ENDIF
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
   \caption{Update with Direct-Mapped LRU Cache}
   \label{alg:cpu-dm-lru}
\begin{algorithmic}
   \STATE {\bfseries Input:} embedding $T$, tag indices $I_C$ of cached rows, indices to update $I_U$, hash function $h$, gradient update $U$
   \FOR{$i$ in $I_U$}
   \IF{$i ==  I_C[h(i)]$}
   \STATE apply gradient updates $T[i,:] \gets T[i,:] + U[i,:]$
   \ELSE 
   \STATE dequantize $T[i,:]$ (which is a no-op) 
   \STATE apply $T[i,:] \gets T[i,:] + U[i,:]$
   \STATE evict index $j = I_C[H(i)]$ by
   \STATE (1) fake quantize $T[j,:]$ and (2) $I_C[h(i)] \gets i$
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
   \caption{Update with Set-Associative LFU Cache}
   \label{alg:cpu-assoc-lfu}
\begin{algorithmic}
   \STATE {\bfseries Input:} embedding $T$, sets of indices $I_C$ of current cached rows, indices to update $I_U$, hash function $h$, gradient update $U$, access counters $Q$ 
   \FOR{$i$ in $_U$}
   \STATE $Q[i] = Q[i] + 1$
   \IF{$i \in I_C[h(i)]$}
   \STATE apply gradient updates $T[i,:] = T[i,:] + U[i,:]$
   \ELSE 
     \STATE dequantize $T[i,:]$ (an no-op)
     \STATE and apply gradient updates $T[i,:] = T[i,:] + U[i,:]$
     \STATE get $s \gets h(i)$, 
     \STATE and $j$ such that $Q[j] = \min\{Q[k] | k \in I_C[s]\}$
     \IF{$Q[i] \le Q[j]$} 
     \STATE quick bypass as follows
     \STATE fake quantize $T[i,:]$
     \ELSE 
     \STATE fake quantize $T[j,:]$
     \STATE replace $j$ by $i$ in the set $I_C[s]$
     \ENDIF
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}


==> placeholder.tex <==
\section{Place Holder}\label{sec:dummy}

A tentative outline
\begin{enumerate}
    \item Introduction: The efficacy and importance of embeddings; big models often have huge tables; numerous work try to reduce the size of these tables without sacrificing accuracy; problem is challenging for recommedation models; show architecture of model and how the embedding tables are used in forward pass (inference and training) and backward pass (training); our compression approach here
    \item Related work: compression by factorization -- tensor decomposition, "remainder trick" of Maxim/Michael Shi/Dheevatsa, mixed-dimension Tony/Maxim et. al.; compression by quantization (various people); Other??
    \item Mixed-Precision Embedding with Cache
    \begin{itemize}
        \item Memory reduction by low precision and the general idea of mitigation of precision loss with a full-precision cache
        \item The basic architecture of model with a cache (using DLRM as a representative model). Show how forward and backward pass operate with a cache. Probably good to show the different cases of CPU only and CPU with GPU.
        \item The idea of popular rows and a couple of analytical results on collision probability analysis with different cache architecture and replacement policies.
    \end{itemize}
    \item Implementation (CPU and GPU)
    \item Experiments and Results
    \begin{itemize}
        \item Explain the set up
        \item Results validating accuracy and efficacy of the method proposed here
        \item Performance results
    \end{itemize}
    \item Concluding remarks
\end{enumerate}



==> tbl_gpu_hit_rate.tex <==

\begin{table}[t]
\caption{Cache hit rates for a large dataset on GPUs for varying replacement policies and sizes (relative to embedding tables)}
\label{tab:gpu-cache-stats}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{rcc}
\toprule
  \makecell{Cache Size}  & 32-way LRU & 32-way LFU\\
\midrule
10\% & 59.86\% &	57.31\%  \\
1\%  & 34.72\% & 13.41\% \\
0.1\% & 10.52\%	& 2.41\% \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tbl_gpu_lfu_multi.tex <==
%EXPERIMENTING

\begin{table}[h]
\caption{High-precision LFU cache with varying cache sizes recover accuracy of low-precision embedding tables}
\label{tab:gpu_lfu_multi}
\begin{center}
\begin{scriptsize}    
\begin{sc}
\begin{tabular}{l | c c c c }
\multicolumn{1}{c|}{
\makecell{Cache\\ Size\\ 
\% of}} &
\multicolumn{4}{c}{
\makecell{Accuracy Drop in \% \\ Cache: LFU, multi-table\\
Rounding: \nrnd{Nearest}/\srnd{Stochastic}}
} \\
\multicolumn{1}{c|}{Table} & FP16 & Int8 & Int4 & Int2 \\ \hline

% -0.006	0.001	0.006	0.502	0.023	0.011	0.632	0.045
% 0.003	0.004	0.018	0.083	0.118	0.129	0.891	1.219
% 0.030	0.023	0.747	0.225	0.225	1.453	5.110	6.391
 10\% & \nrnd{-0.006}/\srnd{\bf 0.001} & \nrnd{0.006}/\srnd{0.502} & \nrnd{0.023}/\srnd{0.011} & \nrnd{0.632}/\srnd{0.045} \\
 1\% & \nrnd{\bf 0.003}/\srnd{\bf 0.004} & \nrnd{0.018}/\srnd{\bf 0.083} & \nrnd{0.118}/\srnd{0.129} & \nrnd{0.891}/\srnd{1.219} \\
 0.1\% & \nrnd{\bf 0.030}/\srnd{\bf 0.023} & \nrnd{0.747}/\srnd{\bf 0.225} & \nrnd{0.225}/\srnd{1.453} &\nrnd{5.110}/\srnd{6.391} \\
\end{tabular}
\end{sc}
\end{scriptsize}
\end{center}
%\caption{\Comment{PT: this is a possible replacement for (a) and (b) of Figure 4. It has more precision and perhaps outline the trend better}}
\end{table}


==> tbl_gpu_lru_multi.tex <==
%EXPERIMENTING

\begin{table}[h]
\caption{High-precision LRU cache with varying cache sizes recover accuracy of low-precision embedding tables [TO BE updated]}
\label{tab:gpu_lru_multi}
\begin{center}
\begin{scriptsize}    
\begin{sc}
\begin{tabular}{l | c c c c }
\multicolumn{1}{c|}{
\makecell{Cache\\ Size\\ 
\% of}} &
\multicolumn{4}{c}{
\makecell{Accuracy Drop in \% \\ Cache: LRU, multi-table\\
Rounding: \nrnd{Nearest}/\srnd{Stochastic}}
} \\

%-0.007	0.003	0.007	0.000	0.012	0.594	0.035	0.048
%0.006	-0.006	0.005	0.604	0.807	0.117	1.507	0.999
%0.033	0.025	3.148	0.461	3.580	2.019	4.062	3.870

\multicolumn{1}{c|}{Table} & FP16 & Int8 & Int4 & Int2 \\ \hline
 10\% & \nrnd{-0.007}/\srnd{0.003} & \nrnd{0.007}/\srnd{	0.000} & \nrnd{0.012}/\srnd{\textunderscore{0.594}} & \nrnd{0.035}/\srnd{0.048} \\
1\% & \nrnd{0.006}/\srnd{-0.006} & \nrnd{0.005}/\srnd{0.604} & \nrnd{0.807}/\srnd{0.117} & \nrnd{1.507}/\srnd{0.999} \\
0.1\% & \nrnd{0.033}/\srnd{0.025} & \nrnd{3.148}/\srnd{0.461} & \nrnd{3.580}/\srnd{2.019} & \nrnd{4.062}/\srnd{3.870} \\
\end{tabular}
\end{sc}
\end{scriptsize}
\end{center}
%\caption{\Comment{PT: this is a possible replacement for (a) and (b) of Figure 4. It has more precision and perhaps outline the trend better}}
\end{table}


==> tmp_tbl.tex <==
EXPERIMENTING

\begin{table}[h]
\begin{tabular}{l | c c c c }
\multicolumn{1}{c|}{
\makecell{Cache\\ Size\\
\% of}} &
\multicolumn{4}{c}{
\makecell{Accuracy Drop in \% (smaller, better)\\ Cache: LRU, Direct Map\\
Rounding: \nrnd{Nearest}/\srnd{Stochastic}}
} \\
\multicolumn{1}{c|}{Table} & int2 & int4 & int8 & FP16 \\ \hline
 0\% & \nrnd{1.4}/\srnd{1.5} & \nrnd{0.6}/\srnd{1.1} & \nrnd{0.5}/\srnd{0.1} & \nrnd{0.1}/\srnd{0.0} \\
 10\% & \nrnd{1.4}/\srnd{1.5} & \nrnd{0.6}/\srnd{1.1} & \nrnd{0.5}/\srnd{0.1} & \nrnd{0.1}/\srnd{0.0}
\end{tabular}
\caption{\Comment{PT: this is a possible replacement for (a) and (b) of Figure 4. It has more precision and perhaps outline the trend better}}
\end{table}

